Controller synthesis for MDPs and Frequency LTL$\setminus$GU

Quantitative extensions of temporal logics have recently attracted significant attention. In this work, we study frequency LTL (fLTL), an extension of LTL which allows to speak about frequencies of events along an execution. Such an extension is particularly useful for probabilistic systems that often cannot fulfil strict qualitative guarantees on the behaviour. It has been recently shown that controller synthesis for Markov decision processes and fLTL is decidable when all the bounds on frequencies are 1. As a step towards a complete quantitative solution, we show that the problem is decidable for the fragment fLTL$\setminus$GU, where U does not occur in the scope of G (but still F can). Our solution is based on a novel translation of such quantitative formulae into equivalent deterministic automata.

==> preliminaries.tex <==
\section{Preliminaries}
\vojta{vzato z nasi LICS/CONCUR submission}
We now proceed with introducing basic notions we use throughout this paper.

A {\em probability distribution} over a finite or countable set $X$ is a function $d : X \to [0,1]$ such that
$\sum_{x\in X} d(x) = 1$, and $\dist(X)$ denotes the set of all probability distributions over $X$.

\mypara{Markov decision processes and Markov chains}
A {\em Markov decision process} (MDP) is a tuple $\mdp = (\states, \actions, \tra)$ where $\states$ is a finite set of states,
$\actions$ is a finite set of actions, and $\tra:\states\times\actions\rightarrow \dist(S)$
is a partial probabilistic transition function.
A {\em Markov chain} (MC) is an MDP in which for every $s\in \states$ there is exactly one $a$ with
$\tra(s,a)$ being defined. We omit actions completely when we speak
about Markov chains and no confusion can arise.

An infinite {\em path}, also called \emph{run}, in $\mdp$ is a sequence $\omega = s_0a_0s_1a_1\cdots$ of states and actions
such that $\tra(s_i,a_i)(s_{i+1}) > 0$ for all $i$, and we denote by $\omega(i)$ the suffix $s_ia_is_{i+1}a_{i+1}\cdots$.
A finite path $h$, also called \emph{history}, is a prefix of an infinite path
ending in a state. 
%
Given a finite path $h=s_0a_0s_1a_1\cdots s_i$ and a finite or infinite path $h'=s_ia_is_{i+1}a_{i+1}\cdots$
we use $h\cdot h'$ to denote the concatenated path $s_0a_0s_1a_1\cdots$.
%
The set of paths starting with a prefix $h$ is denoted by $\cyl(h)$, or simply by $h$ if it leads to no confusion.
We overload the notation also for sets of histories, we simply use $H$ instead of $\bigcup_{h\in H} \cyl(h)$.
%
%

A {\em strategy} is a function $\sigma$ that to every finite path $h$ assigns a probability distribution over actions such that
if an action $a$ is assigned a non-zero probability, then $\tra(s,a)$ is defined where $s$ denotes the last state in $h$. A strategy $\sigma$ is {\em deterministic} if it assigns
Dirac distribution to any history, and {\em randomised} otherwise. Further, it is {\em memoryless} if its choice only depends on
the last state of the history, and {\em finite-memory} if there is a finite automaton such that $\sigma$ only makes its choice based on
the state the automaton ends in after reading the history.

An MDP $\mdp$, a strategy $\sigma$ and an initial state $s_{in}$ give rise to a probability space $\Prb[s_{in}]\sigma$ defined in a standard way~\cite{KSK76}. For a history $h$ and a measurable set of runs $U$ starting from the last state of $h$, we denote by $\Prb[h]{\sigma}(U)$ the probability
$\Prb[s_{in}]{\sigma}(\{h\cdot\omega \mid \omega \in U \} \mid h)$.
Similarly, for a random variable $X$ we denote by $\Ex[s_{in}]{\sigma}{X}$ the expectation of $X$ in this probability space and by $\Ex[h]{\sigma}{X}$ the expectation $\Ex[s_{in}]{\sigma}{X_h \mid h}$. Here, $X_h$ is defined by $X_h(h\cdot\omega) = X(\omega)$ for runs of the form $h\cdot \omega$, and by $X_h(\omega') = 0$ for all other runs.
%
%
%
We say that a property holds {\em almost surely} (or for almost all runs, or almost every run)
if the probability of the runs satisfying the property is $1$.

%
%
%

\mypara{Frequency LTL}
%
The syntax of {\em frequency LTL (fLTL)} is defined by the equation:
\[
 \varphi ::= \alpha \mid \neg \varphi \mid \varphi \vee \varphi \mid \X \varphi \mid \varphi \U \varphi \mid \Gf{p} \varphi
\]
where $\alpha$ ranges over a set $\mathit{AP}$ of atomic propositions. The logic LTL is obtained by omitting the rule for
$\Gf{p} \varphi$.
%
For Markov chains we study the whole fLTL whereas for MDP, we restrict to a fragment that we call \emph{1-fLTL}. In this fragment, negations only occur immediately preceding atomic propositions, and $\Gf{p}$ operators occur only with $p=1$.

For an infinite sequence
$\gamma=x_1x_2\ldots$ of numbers, we set $\freq{\gamma} := \liminf_{i\to \infty} \frac{1}{i} \sum_{j=1}^i x_i$.
%
Given a valuation $\nu : S \rightarrow 2^\mathit{AP}$, the semantics of fLTL is defined over a path $\omega = s_0a_0s_1\dots$ of an MDP as follows.
\[
{%
\begin{array}{llll}
 \omega\models \alpha &\text{iff } \alpha\in \nu(s_0)&
 \ \omega\models \X \varphi &\text{iff } \omega(1) \models\varphi\\
 \omega\models \neg \varphi &\text{iff } \omega \not\models\varphi&
 \ \omega\models \varphi_1\U\varphi_2 &\text{iff } \exists k : \omega(k) \models\varphi_2 \wedge \forall \ell{<}k : \omega(\ell) \models \varphi_1\\
 \omega\models \varphi_1 {\vee} \varphi_2 &\text{iff } \omega {\models}\varphi_1\text{ or }\omega{\models}\varphi_2&
 \ \omega\models \Gf{p}\varphi &\text{iff } \freq{\idf_{\varphi,0}\idf_{\varphi,1}\ldots} \ge p\\
\end{array}
}
\]
where $\idf_{\varphi,i}$ is $1$ for $\omega$ iff $\omega(i) \models \varphi$, and $0$ otherwise.
%
We define $\true, \false$, $\wedge$, and $\rightarrow$ by their usual definitions and introduce standard operators
$\F$ and $\G$ by putting $\F\varphi \equiv \true \U \varphi$ and
$\G\varphi \equiv \neg \F \neg \varphi$. 
%
Finally, we use $\Pr{\sigma}{\varphi}$ as a shorthand for $\Pr{\sigma}{\{\omega \mid \omega\models \varphi\}}$.
\jena{Mozna chceme mit explicitne $G^{\geq p}$ a $G^{< p}$ atd.}
The \fltlfragment{} fragment of fLTL that we study in this paper is defined by disallowing TODO\vojta{doplnit}.

\begin{definition}[Controller synthesis]
The controller synthesis problem asks to decide, given an MDP $\mdp$, a valuation $\nu$, an initial state $\sinit$, an fLTL formula $\varphi$ and
a probability bound $x$, whether
$\Pr[\sinit]{\sigma}{\varphi} \ge x$ for some strategy $\sigma$.
\end{definition}

